Improving Dialog Evaluation with a Multi-reference Adversarial Dataset and Large Scale Pretraining

There is an increasing focus on model-based dialog evaluation metrics such as ADEM, RUBER, and the more recent BERT-based metrics. These models aim to assign a high score to all relevant responses and a low score to all irrelevant responses. Ideally, such models should be trained using multiple relevant and irrelevant responses for any given context. However, no such data is publicly available, and hence existing models are usually trained using a single relevant response and multiple randomly selected responses from other contexts (random negatives). To allow for better training and robust evaluation of model-based metrics, we introduce the DailyDialog++ dataset, consisting of (i) five relevant responses for each context and (ii) five adversarially crafted irrelevant responses for each context. Using this dataset, we first show that even in the presence of multiple correct references, n-gram based metrics and embedding based metrics do not perform well at separating relevant responses from even random negatives. While model-based metrics perform better than n-gram and embedding based metrics on random negatives, their performance drops substantially when evaluated on adversarial examples. To check if large scale pretraining could help, we propose a new BERT-based evaluation metric called DEB, which is pretrained on 727M Reddit conversations and then finetuned on our dataset. DEB significantly outperforms existing models, showing better correlation with human judgements and better performance on random negatives (88.27% accuracy). However, its performance again drops substantially, when evaluated on adversarial responses, thereby highlighting that even large-scale pretrained evaluation models are not robust to the adversarial examples in our dataset. The dataset and code are publicly available.

==> discussion_analysis.tex <==
\section{Analysis and Discussions}
In this section we point out some observations on DEB, after analyzing its embeddings and predictions. We also discuss about the specially crafted adversarial negative examples and verify if our initial hypothesis on the potential traps for a model based dialogue evaluator are indeed the ones that fool the model.

\subsection{DEB: Conicity analysis}
We follow \newcite{DBLP:conf/acl/TalukdarSC18conicity} to understand the projections of the positive and negative responses in the embedding space. We find that ADEM has a less spread, even when trained on the dataset. BERT seems to inherently spread out the embeddings of the classes provided to it. We present these findings in table \ref{tab:conicity_bert} and illustrate in Figure . We find the conicity of all the DailyDialog++ embeddings is 0.59 with \{positive responses + random negatives\} and 0.74 with \{positives + adversarial negatives\}. Considering each context at a time, we find that the 5 positive response embeddings are projected a into tight cone on average. Similarly, the 5 negative responses have high conicity, however, the cone corresponding to random negative is well separated from the positive cone and the adversarial negatives cone is confusingly close to the positive embeddings. Since the adversarial negatives are close to the positive responses in the embedding space, these are the natural hard negatives that can be used for triplet loss training. We conduct such experiment and find that the model tends to overfit to the data with such training as evident from the drastic drop in performance on the random negatives. However, on presenting the dataset for training with just the cross-entropy loss, DEB is able to separate the embeddings to achieve a conicity of 0.35 and 0.37 respectively. \\
Here should we write the points that this high conicity might be causing BERT to get too confident on its predictions, i.e., makes predictions close to 0 or 1?
%BERT finetuned on DailyDialog++ with random negatives gets a conicity of xx. However, the adversarial negatives are also mapped very close to the positive responses in this case. (some numbers and metrics to back this claim - cos sim of avgs and conicity). The adversarial negatives finetuned BERT has the following characteristics in embeddings. (take from excel sheet).

%Since the adversarial negatives are close to the positive responses in the embedding space, these are the natural hard negatives that can be used for triplet loss training. We conduct such experiment and find that the model tends to overfit to the data with such training as evident from the drastic drop in performance on the random negatives.\\
% \subsection{DailyDialog++: Visualizing what trips the model in case of adversarial negatives}
% All the current model based evaluation metrics are fooled by our adversarial negatives. We use integrated gradients to get the attributions to the subwords which contributed to the positive class classification of an adversarial negative instance. For this purpose, we employ the technique of integrated gradients for the attributions and present some examples as in Figure \ref{fig:int_rand_negs}.

% \begin{figure*}
%     \centering
%     \includegraphics[width=1.0\textwidth]{figures/random_neg_integrated.png}
%     \caption{Sub-word attributions for a context with an adversarial negative response}
%     \label{fig:int_rand_negs}
% \end{figure*}

%TODO: write a little bit about integrated gradients. Get better examples and better images.
% TODO in this section:
% \begin{itemize}
%     \item Conicity analysis - clean write up, add visualization
%     %\item Triplet Loss (while training with negatives on BERT and RUBER)
%     %\item Compute the average distance between the embeddings of the positive and negative examples for ADEM, RUBER, Our model [for our model you will take the embedding fed to the next sentence classifier as the final embedding]. Can we also have a t-SNE plot for this.\\ (computing intra and inter-cluster distances between the two clusters (correct references being one cluster and incorrect references being another))
%     \item Integrated Gradients
% \end{itemize}




% \subsection{More works as per time}
% \begin{itemize}
%     \item Obtain model responses from some dialogue models - (might need some human involvement)
%     \item Notes on a BERT-Large model
%     \item Ranking experiments [this will lead to some qualitative analysis] - (will need humans)
%     \item Evaluate the evaluator on Holl-E or other dialogue datasets - (might need humans)
%     \item Fluency tests on some of the variants of attack analysis (such as jumbled stmts) - check perplexity GPT and check BERT scores on these
%     \item Check if originally the adversarial negatives were closer to the positives (in the reddit pretrained/daily with random negatives finetuned models) - checked, works fine - based on conicity, need to write properly, can motivate dataset and triplet loss using this.
%     \item check delta BLEU?
%     \item provide some part of the context itself as a response
%     \item jumble some key words from the context
% \end{itemize}

==> dump.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{|L{4cm}|C{2.3cm}|C{2.3cm}|C{2.3cm}|}
    \hline
         Modification & bert-best & ruber-best &bert-adv \\
         \hline
         Original (for comparison) & \colorbox{springbud}{5117} \colorbox{palerobineggblue!70}{\ 583\ }
 \colorbox{pastelyellow!70}{\ 254\ } \colorbox{wildwatermelon!80}{5446} & \colorbox{springbud}{5067}\     \ \colorbox{palerobineggblue!70}{\ 633\ }
 \colorbox{pastelyellow!70}{1205} \colorbox{wildwatermelon}{4495} &  [[\colorbox{springbud}{4718}  982]
 [1065 \colorbox{orange!70}{4635}]] \\
         \hline
         jumble & \colorbox{springbud}{3951} \colorbox{palerobineggblue!70}{1749}
  \colorbox{pastelyellow!70}{\ 770\ } \colorbox{wildwatermelon}{4930} & \colorbox{springbud}{4683} \colorbox{palerobineggblue!70}{1017}
 \colorbox{pastelyellow!70}{1406} \colorbox{wildwatermelon}{4294} & \colorbox{springbud}{2664} \colorbox{pastelyellow}{3036}
  \colorbox{pastelpink}{844} \colorbox{wildwatermelon}{4856} \\ 
         \hline
         reverse & \colorbox{springbud}{3405} \colorbox{palerobineggblue!70}{2295}
 \colorbox{pastelyellow!70}{\ 680\ } \colorbox{wildwatermelon}{5020} &  \colorbox{springbud}{5317}  \colorbox{palerobineggblue!70}{\ 383\ }
 \colorbox{pastelyellow!70}{2440} \colorbox{wildwatermelon!80}{3260}  & \colorbox{springbud}{1998} 3702
 \colorbox{pastelyellow!70}{\ 635\ } \colorbox{wildwatermelon}{5065}\\ 
         \hline
         no stopwords & \colorbox{springbud}{4891}\  \colorbox{palerobineggblue!70}{\ 809\ }
 \colorbox{pastelyellow!70}{\ 671\ } \colorbox{wildwatermelon}{5029}\  \underline{pearson=.58} & \colorbox{springbud}{4520}\ \colorbox{palerobineggblue!70}{1180}
 \colorbox{pastelyellow!70}{1307} \colorbox{wildwatermelon}{4393} pearson=.52 & \colorbox{springbud}{4284}\ \colorbox{pastelyellow!70}{1416}
 \colorbox{pastelyellow!70}{1329} \colorbox{wildwatermelon}{4371} \underline{pearson=.52}\\ 
         \hline
         no punctuation & \colorbox{springbud}{4922}  \colorbox{palerobineggblue!70}{\ 778\ }
 \colorbox{pastelyellow!70}{\ 219\ } \colorbox{wildwatermelon}{5481}  & \colorbox{springbud}{5306}  \colorbox{palerobineggblue!70}{\ 394\ }
 \colorbox{pastelyellow!70}{2447} \colorbox{wildwatermelon}{3253} &  [[4235 1465]
 [831 4869]]  \\ 
         \hline
         Replacing with synonyms &\colorbox{springbud}{4630} \colorbox{palerobineggblue!70}{1070}
 \colorbox{pastelyellow!70}{\ 298\ } \colorbox{wildwatermelon}{5402} pearson=.676 & \colorbox{springbud}{5073}\colorbox{palerobineggblue!70}{\ 627\ }
 \colorbox{pastelyellow!70}{1867} \colorbox{wildwatermelon}{3833} pearson=.43 & [[4246 1454]
 [995 4705]] pearson=.58\\ 
         \hline
         Retain only nouns & \colorbox{springbud}{3428} \colorbox{palerobineggblue!70}{2272}
 \colorbox{pastelyellow!70}{1197} \colorbox{wildwatermelon}{4503}  & \colorbox{springbud}{4729}  \colorbox{palerobineggblue!70}{\ 971\ }
 \colorbox{pastelyellow!70}{4403} \colorbox{wildwatermelon}{1297}  &  [[2760 2940]
 [1403 4297]] \\
         \hline
         Retain only nouns, pronouns and verbs & \colorbox{springbud}{4293} \colorbox{pastelyellow!70}{1407}
 \colorbox{pastelyellow!70}{\ 771\ } \colorbox{wildwatermelon}{4929}  & \colorbox{springbud}{4803} \colorbox{palerobineggblue!70}{\ 897\ }
 \colorbox{pastelyellow!70}{2489} \colorbox{wildwatermelon}{3211} & [[3092 2608]
 [1086 4614]] 67.5\%\\
         %with random negatives & & \\
         
         %with adv. negatives & & \\
         %\hline
         %BERT finetuned using both$^*$ &88.67 &92.65 \\
         %hard and random negatives$^*$ & & \\
         \hline
    \end{tabular}
    \caption{Modifying the dataset with an aim to confuse the model and check its robustness}
    \label{tab:attacks}
\end{table*}

==> extra_stuff.tex <==
\section{Extra stuff}
The remaining stuff below will move to appropriate sections/subsections above. 

In this section, we first compare various evaluation metrics described in sections \ref{sec:existing-metrics} and \ref{sec:DEB}. The idea is to check whether having multiple relevant references improves the performance of trained and untrained metrics. To begin with, we limit our analysis to multiple relevant responses and random negative responses. In later sub-sections we also check the performance in the presence of adversarial examples and show how such examples affect the performance of trained metrics. Following this, in the next section we do a detailed ablation study and analysis of DEB and compare it closely with ADEM and RUBER. 

%We first evaluate using random negatives as irrelevant responses which is the approach taken by all the existing studies on the dialogue evaluation methods. We find that BERT-based dialogue evaluation model, \textit{DEB}, achieves the best accuracy and correlation with human judgements. We then try to attribute the performance of DEB to its various stages of training through ablation studies. 

%\subsection{Ablation studies}
%The trained models perform well on identifying the relevant and irrelevant responses. However, this is as per the expectation from these models of high capacity, after being trained for the task specifically. In this section we take a closer look at the contributions of the different stages of training these models by evaluating the models at each juncture with the mutlireference DailyDialog++ with random negatives. BERT model when adopted directly for the task of dialog evaluation gives 72.6\% accuracy. It has a high false positive percentage with more than 52\% of the negatives getting classified as positives. %with most of the error due to false positives.
BERT performs better when pretrained with Reddit data and achieves 84.2\% on DailyDialog++ even without seeing any training instance from this dataset. Only 26\% of the negatives are falsely classified as positives in this case. This shows that dialogue evaluation task specific pretraining using large-scale dialogue datasets boosts the performance significantly. Finetuning BERT on DailyDialog++ with one pass over the dataset with a learning rate of $1e^-5$ further improves the accuracy to 88.3\%.
%BERT performs better when pretrained with Reddit data, however the adversarial negatives trip the model, with most of them being wrongly classified as positive/true responses. We provide the confusion matrices of the model predictions on the test set in Table \ref{tab:bert_conf}. %(Should we present only BERT confusion in this table or have RUBER also? Similar) 
%Finetuning BERT on DailyDialog++ with random negatives still does not improve its susceptibility to adversarial negatives much. However, finetuning it with the adversarial negatives helps in boosting performance without any significant drop in performance on random negative, unlike in case of RUBER. The best results are when the model is trained using both adversarial and random negatives. All the above experiments' results are tabulated in Table \ref{tab:accuracies}.

Since the dataset is human-curated, we can study the correlation of the models with human judgement. We employ point-biserial correlation since the human decisions on the responses on our dataset are binary whereas the models can be probed for real-valued scores, before converting them to binary decisions, if at all.  (rephrase this, TODO: pending - to report/refer to these correlations in table.)
% ADEM:\\
% pretraining the VHRED using reddit data (probably need not do pretraining here. The parameters to be learnt are just the matrices used in the scoring function. Also the VHRED training by the original authors Twitter data should be as good as Reddit)\\
% TODO: Finetuning using (i) random negatives (ii) hard negatives (iii) both\\
% Results of the above 3 finetuned models on only random negative sampled data and hard negative data, along with results before any finetuning at all (i.e., original ADEM model)\\
% \newline RUBER:\\ We will pretrain it with Reddit data. Then finetune and report results same as above.

% Human verifications:\\
% Usage of random samples in training these models - basically wrong or right? 
% (Get the percentage of random negatives becoming right "by-chance" through human evaluation on a small sample)\\

%\newline BERT : similar experiments as above. Probably all these results will go into a few big tables.\\

% \begin{table}[t]
%  \caption{The confusion matrix}
%  \label{tab:CM}
%     \centering
%     \resizebox{1\textwidth}{!}{ % to nicely resize the table in the text width

%   \begin{tabular}{r*{6}{G}}
%   \rotz{} & 
%   \rotz{A} & 
%   \rotz{B} & 
%   \rotz{C} &
%   \rotz{D} & 
%   \rotz{E} \smallskip \\ 
%   A        & 0.54  & 0     & 0.08  & 0.17  & 0     \\ 

%   B        & 0     & 0.96  & 0     & 0     & 0     \\ 

%   C        & 0.04  & 0.04  & 0.38  & 0.13  & 0     \\ 

%   D        & 0.08  & 0     & 0.04  & 0.75  & 0     \\ 

%   E        & 0     & 0.04  & 0     & 0     & 0.96  \\ 

%   \end{tabular}%\par\bigskip
%   }
% \end{table}

% ('Conicity of all the embeddings considered:', 0.5855594193026792)

% ('Avg of conicity of positives (an instance at a time):', 0.8896663521523488)
% ('Avg of conicity of negatives (an instance at a time):', 0.8342379562581723)
% ('Avg of conicity of all responses for a context:', 0.621718516752763)
% 1141
% ('Avg cosine similarity between positive emb mean and neg embedding mean:', 0.037269361677595356)
% ('Min cosine sim:', -0.840187116700311)
% ('Max cosine sim::', 0.9912561299067881)
% ('Mean of mean of response embeddings for a context:', -0.012884779160159012)
% ('Conicity of mean of response embeddings for a context:', 0.9277125125393835)
% ('Conicity of all positives:', 0.8248009594494184)
% ('Conicity of all negatives:', 0.7755089427077063)



%TODO : Losses here \\

%\subsection{Hand crafted attacks}
%We also aim to understand the robustness of these models in case of other adversarial conditions. Towards this end, we employ the attacks suggested in \newcite{DBLP:conf/aaai/SaiGKS19Reeval} involving modifications to the data. These results are presented in Table \ref{tab:attacks}. The modifications of jumbling and reversing the words in a response make it irrelevant and hence we expect to see more of the original true positives get classified as negatives. DEB does this better than the RUBER model. Similar is the case with the drastic change of retaining only nouns in a response. For the modifications of removing stopwords and replacing some of the words in the response with their  synonyms using wordnet, we perform human evaluations. We present humans with these modified responses for the context and obtain scores in the range 0 to 3, higher score meaning better response. We consider human scores on 400 samples for this task and compute the pearson correlation of the model predictions with the human judgements. In this case, we find DEB is better correlated with human judgements on both the modifications. For punctuation removal, we don't expect drastic change and the models perform as expected.
%(should we move this to next section?)
%Attacks - how do each of these perform when words are jumbled, (other modifications and attacks)

%\subsection{Adversarial Evaluation on DailyDialog++}
%BERT trained with the popular technique of random matching for negative references works well on evaluating similar data. However, the adversarial negatives trip the model, with most of them being wrongly classified as positive/true responses. We provide the confusion matrices of the model predictions on the test set in Table \ref{tab:bert_conf}. However, if the model is exposed to the adversarial instances during training, it learns to distinguish between the positives and adversarial negatives. The best results are when the model is trained using both adversarial and random negatives.\\
%1. ADEM, RUBER, DEB are bad.  - put confusion matrix on trained on rand negs - put acc and pbc nos only (no box plot)\\
%2. say if it's trained on both eg, it improves - just pbc and acc numbers 

%\subsection{Different loss functions for training DEB}


%Since the adversarial negatives are close to the positive responses in the embedding space, these are the natural hard negatives that can be used for triplet loss training. We conduct such experiment and find that the model tends to overfit to the data with such training as evident from the drastic drop in performance on the random negatives. However, on presenting the dataset for training with just the cross-entropy loss, DEB is able to separate the embeddings to achieve a conicity of 0.35 and 0.37 respectively.
%BERT seems to inherently spread out the embeddings of the classes provided to it. We present these findings in table \ref{tab:conicity_bert} and illustrate in Figure . We find the conicity of all the DailyDialog++ embeddings is 0.59 with \{positive responses + random negatives\} and 0.74 with \{positives + adversarial negatives\}. Considering each context at a time, we find that the 5 positive response embeddings are projected a into tight cone on average. Similarly, the 5 negative responses have high conicity, however, the cone corresponding to random negative is well separated from the positive cone and the adversarial negatives cone is confusingly close to the positive embeddings. Since the adversarial negatives are close to the positive responses in the embedding space, these are the natural hard negatives that can be used for triplet loss training. We conduct such experiment and find that the model tends to overfit to the data with such training as evident from the drastic drop in performance on the random negatives. However, on presenting the dataset for training with just the cross-entropy loss, DEB is able to separate the embeddings to achieve a conicity of 0.35 and 0.37 respectively. \\
%Here should we write the points that this high conicity might be causing BERT to get too confident on its predictions, i.e., makes predictions close to 0 or 1?

==> full_table.tex <==
\begin{table}[t]
        \centering
        \resizebox{1.0\columnwidth}{!}{
        \begin{tabular}{|c|c|c|}
        \hline
         Model & Rand Neg & Adv Neg\\
         \hline
         \cite{shimanaka19} finetuned on rand neg & 73.40  & 67.57 \\ 
         \cite{shimanaka19} finetuned on adv. neg & 69.89  & 75.92 \\ 
         \cite{shimanaka19} finetuned on both & 72.77 & 74.55 \\ 
         \hline
         \cite{ghazarian19} trained on rand neg & 74.67 & 60.14 \\
         \cite{ghazarian19} trained on adv. neg &  60.49 & 87.67 \\
         \cite{ghazarian19} trained on both & 73.87 & 86.61\\ \hline
         RUBER pretrained on Reddit & 72.18  & 55.75 \\ 
         Pretrained RUBER finetuned on rand neg & 78.18  & 64.96 \\ 
         Pretrained RUBER finetuned on adv. neg & 70.82  & 76.5 \\ 
         Pretrained RUBER finetuned on both & 75.11  & 83.88 \\ 
         \hline
         BERT original & 72.65  & 58.10 \\ 
         DEB pretrained on Reddit & 84.16 & 59.82 \\
         Pretrained DEB finetuned on rand neg & 88.29 & 66.75 \\
         %with random negatives & & \\
         Pretrained DEB finetuned on daily on adv. neg & 86.24 & 82.04 \\
         % & & \\
         Pretrained DEB finetuned on both &\textbf{88.67} &\textbf{92.65} \\   
             %hard and random negatives$^*$ & & \\
             \hline
             %\hline
             %Other losses & & \\
             %\hline
             %DEB with hinge loss & 80.65\%  & 90.33\% \\
             %BERT with hinge loss & 76\%  & 95.6\% \\
             %\hline
             %DEB with triplet loss & 66.82\% & 82.75\% \\
             %\hline
        \end{tabular}
        }
        \caption{Performance of DEB and RUBER variants.}
        \label{tab:accuracies}
    \end{table}

==> table_adv_size.tex <==
\begin{table}[t]
\centering
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{|C{2.5cm}|c|c|c|}
\hline
        \% of adversarial examples added & Adv neg & Positive & Rand neg \\\hline
         0 & 45.60 & 87.91 & 88.67\\
         1 & 70.85 & 84.31 & 90.05 \\
         10 & 83.16 & 86.54 & 88.21\\
         50 & 90.08 & 88.96 & 86.16\\
         75 & 93.04 & 89.37 & 86.71\\
         100 & 95.54 & 89.77 & 87.58\\
         %(on more iterations/overfitting) & 95.54 & 89.77 & 87.58\\
         \hline
   \end{tabular}}
\caption{Effect of varying the amount of adversarial negatives added to the training set.}
% All the adversarial negative instances in the training set are seen only once by the model in all the above cases except the last.
\label{tab:adv_size}
\end{table}

==> table_attack.tex <==
\setlength{\tabcolsep}{13pt}
\renewcommand{\arraystretch}{1.0}
\begin{table*}[h]
    \centering
    \begin{tabular}{|L{3cm}|C{2.3cm}|C{2.3cm}|C{2.5cm}|}
    \hline
    %\cline{1-3}
         Modification & DEB-best & RUBER-best & observations \\
         \hline
         %\cline{1-3}
         Unmodified (for comparison) & \colorbox{springbud}{5117} \colorbox{palerobineggblue!70}{\ 583\ }
 \colorbox{pastelyellow!70}{\ 254\ } \colorbox{wildwatermelon}{5446} & \colorbox{springbud}{5067}\     \ \colorbox{palerobineggblue!70}{\ 633\ }
 \colorbox{pastelyellow!70}{1205} \colorbox{wildwatermelon}{4495} & \colorbox{springbud}{TP} \colorbox{palerobineggblue}{FN}\newline
 \colorbox{yellow!70}{FP} \colorbox{wildwatermelon}{TN} \\
         %\cline{1-3}
         \hline
         jumble & \colorbox{springbud}{3951} \colorbox{palerobineggblue!70}{1749}
  \colorbox{pastelyellow!70}{\ 770\ } \colorbox{wildwatermelon}{4930} & \colorbox{springbud}{4683} \colorbox{palerobineggblue!70}{1017}
 \colorbox{pastelyellow!70}{1406} \colorbox{wildwatermelon}{4294} & \multirow{3}{3cm}{Candidates originally classified as positives become negatives}\\
         \cline{1-3}
         reverse & \colorbox{springbud}{3405} \colorbox{palerobineggblue!70}{2295}
 \colorbox{pastelyellow!70}{\ 680\ } \colorbox{wildwatermelon}{5020} &  \colorbox{springbud}{5317}  \colorbox{palerobineggblue!70}{\ 383\ }
 \colorbox{pastelyellow!70}{2440} \colorbox{wildwatermelon!80}{3260}  & \\ 
 \cline{1-3}
         Retain only nouns & \colorbox{springbud}{3428} \colorbox{palerobineggblue!70}{2272}
 \colorbox{pastelyellow!70}{1197} \colorbox{wildwatermelon}{4503}  & \colorbox{springbud}{4729}  \colorbox{palerobineggblue!70}{\ 971\ }
 \colorbox{pastelyellow!70}{4403} \colorbox{wildwatermelon}{1297}  &\\
         \hline %\cline{1-3}
         no stopwords & \colorbox{springbud}{4891}\  \colorbox{palerobineggblue!70}{\ 809\ }
 \colorbox{pastelyellow!70}{\ 671\ } \colorbox{wildwatermelon}{5029}\  \underline{pearson=.58} & \colorbox{springbud}{4520}\ \colorbox{palerobineggblue!70}{1180}
 \colorbox{pastelyellow!70}{1307} \colorbox{wildwatermelon}{4393} pearson=.52 & \multirow{2}{2.8cm}{Good pearson correlation with human judgements} \\ 
 \cline{1-3}
 Replacing with synonyms &\colorbox{springbud}{4630} \colorbox{palerobineggblue!70}{1070}
 \colorbox{pastelyellow!70}{\ 298\ } \colorbox{wildwatermelon}{5402} pearson=.676 & \colorbox{springbud}{5073}\colorbox{palerobineggblue!70}{\ 627\ }
 \colorbox{pastelyellow!70}{1867} \colorbox{wildwatermelon}{3833} pearson=.54 &\\ 
         \hline
         %\cline{1-3}
         no punctuation & \colorbox{springbud}{4922}  \colorbox{palerobineggblue!70}{\ 778\ }
 \colorbox{pastelyellow!70}{\ 219\ } \colorbox{wildwatermelon}{5481}  & \colorbox{springbud}{5306}  \colorbox{palerobineggblue!70}{\ 394\ }
 \colorbox{pastelyellow!70}{2447} \colorbox{wildwatermelon}{3253} &  No major change \\ 
         %\cline{1-3}
         \hline
%          Retain only nouns, pronouns and verbs & \colorbox{springbud}{4293} \colorbox{pastelyellow!70}{1407}
%  \colorbox{pastelyellow!70}{\ 771\ } \colorbox{wildwatermelon}{4929}  & \colorbox{springbud}{4803} \colorbox{palerobineggblue!70}{\ 897\ }
%  \colorbox{pastelyellow!70}{2489} \colorbox{wildwatermelon}{3211} & \\

         %with random negatives & & \\
         
         %with adv. negatives & & \\
         %\hline
         %BERT finetuned using both$^*$ &88.67 &92.65 \\
         %hard and random negatives$^*$ & & \\
         \cline{1-3}
    \end{tabular}
    \caption{Performance of RUBER and DEB on synthetically crafted adversarial responses}
    \label{tab:attacks}
\end{table*}

==> table_attack_backup.tex <==
\setlength{\tabcolsep}{13pt}
\renewcommand{\arraystretch}{1.0}
\begin{table*}[h]
    \centering
    \begin{tabular}{L{4cm}|C{2.3cm}|C{2.3cm}|C{2.3cm}}
    \hline
         Modification & bert-best & ruber-best &bert-adv \\
         \hline
         Original (for comparison) & [[5117  583] 
 [254 \colorbox{richmaroon}{5446}]] 92\% & [[5067  633]
 [1205 4495]] 83.88\% &  [[4718  982]
 [1065 4635]] 82\%\\
         \hline
         jumble & [[3951 1749] 
  [770 4930]] (77.9\%)  & [[4683 1017]
 [1406 4294]] 78.75\% & [[2664 3036]
  [844 4856]] 65.96\\ 
         \hline
         reverse & [[3405 2295]
 [680 5020]] 73.9  &  [[5317  383]
 [2440 3260]] 75.2\% & [[1998 3702]
 [635 5065]] 61.95\%\\ 
         \hline
         no stopwords & [[4891  809]
 [671 5029]] 87\% \underline{pearson=.58} & [[4520 1180]
 [1307 4393]] 78.18\% & [[4284 1416]
 [1329 4371]] 75.9\% \underline{pearson=.52}\\ 
         \hline
         no punctuation & [[4922  778]
 [219 5481]] 91.25\%  & [[5306  394]
 [2447 3253]] 75\% &  [[4235 1465]
 [831 4869]] 79.85\% \\ 
         \hline
         Replacing with synonyms &[[4630 1070]
 [298 5402]] 88\% pearson=.676 & [[5073  627]
 [1867 3833]] 78.12\%  & [[4246 1454]
 [995 4705]] 78.5\% pearson=.58\\ 
         \hline
         Retain only nouns & [[3428 2272]
 [1197 4503]] 69.5\% & [[4729  971]
 [4403 1297]] 52.8\% &  [[2760 2940]
 [1403 4297]] 61.9\%\\
         \hline
         Retain only nouns, pronouns and verbs & [[4293 1407]
 [ 771 4929]] 80.89\% & [[4803  897]
 [2489 3211]] 70.3\% & [[3092 2608]
 [1086 4614]] 67.5\%\\
         %with random negatives & & \\
         
         %with adv. negatives & & \\
         %\hline
         %BERT finetuned using both$^*$ &88.67 &92.65 \\
         %hard and random negatives$^*$ & & \\
         \hline
    \end{tabular}
    \caption{Modifying the dataset to confuse the model/check its robustness}
    \label{tab:attacks}
\end{table*}

==> table_evaluation_adversarial.tex <==
\setlength{\tabcolsep}{13pt}
\renewcommand{\arraystretch}{1.0}
\begin{table*}[]
\centering
\resizebox{1.0\textwidth}{!}{
% \scriptsize{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\multicolumn{1}{l|}{Metric} & \multicolumn{2}{c|}{Positive Scores}               & \multicolumn{2}{c|}{Negative Scores}                & \multicolumn{2}{c|}{PBC}                            & \multicolumn{2}{c}{Accuracy}                       \\ \hline
                             & \multicolumn{1}{l|}{Avg} & \multicolumn{1}{l|}{Max} & \multicolumn{1}{l|}{Avg} & \multicolumn{1}{l|}{Max} & \multicolumn{1}{l|}{Avg} & \multicolumn{1}{l|}{Max} & \multicolumn{1}{l|}{Avg} & \multicolumn{1}{l}{Max} \\ \Xhline{3\arrayrulewidth}
BLEU-1                       & 0.1736                  & 0.2877                   & 0.1177                   & 0.1979                   & 0.3858                   & 0.3846                   & 66.94                    & 65.72                    \\
BLEU-2                       & 0.0436                  & 0.1175                   & 0.008                    & 0.0315                   & 0.3673                   & 0.3654                   & 68.83                    & 70.41                    \\
BLEU-3                       & 0.0152                  & 0.048                    & 0.0012                   & 0.0052                   & 0.2566                   & 0.2378                   & 69.78                    & 72.19                    \\
BLEU-4                       & 0.0059                  & 0.0198                   & 0.0004                   & 0.0018                   & 0.1575                   & 0.1446                   & 70.45                    & 72.68                    \\
METEOR                       & 0.0578                  & 0.0964                   & 0.0579                   & 0.1029                   & -0.0732                  & -0.0029                  & 49.59                    & 46.63                    \\
ROUGE-L                      & 0.1982                  & 0.3183                   & 0.1371                   & 0.223                    & 0.4                      & 0.3948                   & 67.58                    & 67.27                    \\ \hline
Embed Avg                    & 0.8666                  & 0.9083                   & 0.8359                   & 0.8807                   & 0.2903                   & 0.2815                   & 64.3                     & 64.65                    \\
Vec Extr                     & 0.5025                  & 0.5962                   & 0.3988                   & 0.4731                   & 0.5485                   & 0.5592                   & 75.33                    & 74.84                    \\ 
GreedyMatch                  & 0.6909                  & 0.7515                   & 0.6341                   & 0.6844                   & 0.5019                   & 0.4981                   & 72.55                    & 72.02                    \\ \hline
BERTScore                    & 0.8576                  & 0.8787                   & 0.8449                   & 0.8601                   & 0.3952                   & 0.3415                   & 66.22                    & 68.85                    \\ \Xhline{3\arrayrulewidth}
ADEM                         & \multicolumn{2}{c|}{0.5753}                        & \multicolumn{2}{c|}{0.4192}                         & \multicolumn{2}{c|}{0.4183}                         & \multicolumn{2}{c}{66.63}                          \\
RUBER                        & \multicolumn{2}{c|}{0.8415}                        & \multicolumn{2}{c|}{0.2837}                         & \multicolumn{2}{c|}{0.7423}                         & \multicolumn{2}{c}{83.83}                          \\ \hline
BERT (ours)                  & \multicolumn{2}{c|}{0.8925}                        & \multicolumn{2}{c|}{0.0451}                         & \multicolumn{2}{c|}{\textbf{0.8690}}                         & \multicolumn{2}{c}{\textbf{92.66}} \\                        
\end{tabular}}
\caption{Automatic evaluation metrics performance as evaluators when using multi-reference responses dataset. (PBC refers to point-biserial coefficient}
\end{table*}

==> table_evaluation_random_old.tex <==
\setlength{\tabcolsep}{16pt}
\renewcommand{\arraystretch}{1.0}
\begin{table*}[]
\centering
\resizebox{0.8\textwidth}{!}{
% \scriptsize{
\begin{tabular}{l|c|c|c|c|c|c}
\multicolumn{1}{c|}{\multirow{3}{*}{Metric}} & \multicolumn{3}{c|}{Point Biserial Correlation}                                                                           & \multicolumn{3}{c}{Accuracy}                                                                      \\ \cline{2-7} \cline{2-7} \cline{2-7} \cline{2-7} 
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\multirow{2}{*}{Single}} & \multicolumn{2}{c|}{Multiple}                       & \multicolumn{1}{c|}{\multirow{2}{*}{Single}} & \multicolumn{2}{c}{Multiple}                       \\ \cline{3-4} \cline{6-7} 
\multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{}                        & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{l|}{}                        & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c}{Max} \\ \Xhline{3\arrayrulewidth}

BLEU-1 & 0.2589 & 0.4197 & 0.4143 & 60.62 & 68.16 & 68.40 \\ 
BLEU-2 & 0.2176 & 0.3855 & 0.3616 & 59.64 & 68.79 & 68.71 \\ 
BLEU-3 & 0.1417 & 0.2615 & 0.2389 & 58.23 & 68.18 & 67.80 \\ 
BLEU-4 & 0.0847 & 0.1657 & 0.1489 & 57.34 & 67.67 & 67.24 \\ 
METEOR & 0.2320 & 0.3963 & 0.4105 & 59.40 & 68.39 & 67.94 \\ 
ROUGE-L & 0.2325 & 0.4085 & 0.3985 & 59.53 & 67.60 & 67.92 \\ \hline
Embed Avg & 0.2302 & 0.2468 & 0.2262 & 61.21 & 61.44 & 62.87 \\ 
Vec Extr & 0.2387 & 0.3465 & 0.3317 & 59.21 & 63.27 & 63.78 \\ 
GreedyMatch & 0.2377 & 0.3610 & 0.3177 & 60.05 & 63.94 & 65.49 \\ \hline
BERTScore & 0.2868 & 0.3916 & 0.3930 & 61.62 & 66.17 & 67.48 \\
%Shimanaka & 0.2868 & - & - & 73.40 & 66.17 & 67.48 \\
\Xhline{3\arrayrulewidth} \hline
ADEM                  & \multicolumn{3}{c|}{0.3950}                         & \multicolumn{3}{c}{64.74}                          \\
Shimanaka                 & \multicolumn{3}{c|}{0.5019}                         & \multicolumn{3}{c}{73.40}                          \\
RUBER                 & \multicolumn{3}{c|}{0.6406}                         & \multicolumn{3}{c}{78.18}                          \\ 
NAACL'19                 & \multicolumn{3}{c|}{0.6287}                         & \multicolumn{3}{c}{78.35}                          \\\hline
DEB (ours)           & \multicolumn{3}{c|}{\textbf{0.7928}}                         & \multicolumn{3}{c}{\textbf{88.27}} \\               
\end{tabular}}
\caption{Automatic evaluation metrics performance on random negatives (PBC refers to point-biserial coefficient. Column subheading 'Single' refers to experiments using single reference response and 'Avg' and 'Max' are the average and maximum aggregation strategies when using multiple reference responses.}
\label{table:eval_random}
\end{table*}

==> table_vars.tex <==
\begin{table*}[]
\centering
\resizebox{0.9\textwidth}{!}{
% \scriptsize{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\multicolumn{1}{c|}{\multirow{2}{*}{Training variant}} & \multicolumn{2}{c|}{\cite{shimanaka19}}                                                                           & \multicolumn{2}{c|}{\cite{ghazarian19}} &    \multicolumn{2}{c|}{RUBER}  &\multicolumn{2}{c}{DEB}                                                         \\ \cline{2-9} \cline{2-9} \cline{2-9} \cline{2-9} 
\multicolumn{1}{c|}{}     & P+R & P+A  & P+R & P+A  & P+R & P+A  & P+R & P+A                        \\ \cline{3-4} \cline{6-7} 
%\multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{}                        & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{l|}{}                        & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c}{Max} \\ 
\Xhline{3\arrayrulewidth}
%pretrained on Reddit & - & - & - & - & 72.18  & 55.75  \\ 
Using rand neg & 73.40  & 67.57 & 74.67 & 60.14 & 78.18  & 64.96 & 88.29 & 66.75 \\ 
Using adv. neg & 69.89  & 75.92 &  60.49 & 87.67  & 70.82  & 76.5 & 86.24 & 82.04\\ 
Using both & 72.77 & 74.55 & 73.87 & 86.61 & 75.11  & 83.88 &\textbf{88.67} &\textbf{92.65} \\ 
\Xhline{3\arrayrulewidth}
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Other baseline variants for comparison}} & \multicolumn{2}{c}{P+R} & \multicolumn{2}{c}{P+A} & \\ 
\hline
\multicolumn{1}{c}{} & \multicolumn{3}{l|}{BERT original} & \multicolumn{2}{c}{72.65} & \multicolumn{2}{c}{58.10} &\\
\multicolumn{1}{c}{} &\multicolumn{3}{l|}{RUBER pretrained on only Reddit} & \multicolumn{2}{c}{72.18} & \multicolumn{2}{c}{55.75} &\\
\multicolumn{1}{c}{} & \multicolumn{3}{l|}{DEB pretrained on only Reddit} & \multicolumn{2}{c}{84.16} & \multicolumn{2}{c}{59.82} &\\
%BERT original & 72.65  & 58.10 \\
%DEB pretrained on Reddit & 84.16 & 59.82
%      RUBER pretrained on Reddit & 72.18  & 55.75 \\ 

\end{tabular}}
\caption{Performance of models based on the different training schemes. The accuracies are reported on the test set of DialyDialog++ on two types: classifying Positive responses from Random negatives (P+R) and distinguishing Positive responses from Adversarial negatives (P+A). Best accuracies for each training method are in \textcolor{red}{red} for P+R and \textcolor{blue}{blue} for P+A.}
\label{table:testing}
\end{table*}

% \begin{table}[t]
%     \centering
%     \resizebox{1.0\columnwidth}{!}{
%     \begin{tabular}{|c|c|c|}
%     \hline
%      Model & Rand Neg & Adv Neg\\
%      \hline
%      \cite{shimanaka19} finetuned on rand neg & 73.40  & 67.57 \\ 
%      \cite{shimanaka19} finetuned on adv. neg & 69.89  & 75.92 \\ 
%      \cite{shimanaka19} finetuned on both & 72.77 & 74.55 \\ 
%      \hline
%      \cite{ghazarian19} trained on rand neg & 74.67 & 60.14 \\
%      \cite{ghazarian19} trained on adv. neg &  60.49 & 87.67 \\
%      \cite{ghazarian19} trained on both & 73.87 & 86.61\\ \hline
%      RUBER pretrained on Reddit & 72.18  & 55.75 \\ 
%      Pretrained RUBER finetuned on rand neg & 78.18  & 64.96 \\ 
%      Pretrained RUBER finetuned on adv. neg & 70.82  & 76.5 \\ 
%      Pretrained RUBER finetuned on both & 75.11  & 83.88 \\ 
%      \hline
%      BERT original & 72.65  & 58.10 \\ 
%      DEB pretrained on Reddit & 84.16 & 59.82 \\
%      Pretrained DEB finetuned on rand neg & 88.29 & 66.75 \\
%      %with random negatives & & \\
%      Pretrained DEB finetuned on daily on adv. neg & 86.24 & 82.04 \\
%      % & & \\
%      Pretrained DEB finetuned on both &\textbf{88.67} &\textbf{92.65} \\   
%          %hard and random negatives$^*$ & & \\
%          \hline
%          %\hline
%          %Other losses & & \\
%          %\hline
%          %DEB with hinge loss & 80.65\%  & 90.33\% \\
%          %BERT with hinge loss & 76\%  & 95.6\% \\
%          %\hline
%          %DEB with triplet loss & 66.82\% & 82.75\% \\
%          %\hline
%     \end{tabular}
%     }
%     \caption{Performance of DEB and RUBER variants.}
%     \label{tab:accuracies}
% \end{table}

==> table_vars_copy.tex <==
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\begin{table*}[]
\centering
\resizebox{0.99\textwidth}{!}{
% \scriptsize{
\begin{tabular}{l|C{2cm}|C{2cm}|c|c|C{2cm}|C{2cm}|c|c}
%\multicolumn{1}{c|}{\multirow{2}{*}{Training variant}}  & 
\multicolumn{1}{c|}{}  & \multicolumn{4}{c|}{\textbf{Testing on Positive vs Random negatives}}  &\multicolumn{4}{c}{\textbf{Testing on Positive vs Adversarial negatives}} \\ 
%\multicolumn{1}{c|}{\multirow{2}{*}{Training variant}} & \multicolumn{4}{c|}{Positive + Random negatives}                             & \multicolumn{4}{c}{Positive + Adversarial negatives}\\ 
%\cline{2-9} \cline{2-9} \cline{2-9} \cline{2-9} 
\multicolumn{1}{c|}{\textbf{Training variant}}  & \cite{shimanaka19} & \cite{ghazarian19}  & RUBER & DEB  & \cite{shimanaka19} & \cite{ghazarian19}  & RUBER & DEB   \\ \cline{3-4} \cline{6-7} 
%\multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{}                        & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c|}{Max} & \multicolumn{1}{l|}{}                        & \multicolumn{1}{c|}{Avg} & \multicolumn{1}{c}{Max} \\ 
\Xhline{3\arrayrulewidth}
%pretrained on Reddit & - & - & - & - & 72.18  & 55.75  \\ 
Using rand neg & 73.40 & 74.67 & 78.18  & \textcolor{red}{88.29}
& \textcolor{blue}{67.57}  & 60.04  & 64.96 & 66.75 \\ 
Using adv. neg & 69.89  &  60.49  & 70.82 & \textcolor{red}{86.24} 
& 75.92 & \textcolor{blue}{87.67}  & 76.50 & 82.04\\ 
Using both & 72.77 & 73.87 & 75.11 & \textcolor{red}{\textbf{88.67}}
& 74.55 & 86.61  & 83.88 & \textcolor{blue}{\textbf{92.65}} \\ 
\Xhline{3\arrayrulewidth}
\hline
 \multicolumn{3}{c}{\textbf{Other baseline training variants for comparison}} & \multicolumn{2}{c|}{} & \multicolumn{3}{c}{} & \\ 
 %\multicolumn{4}{c}{\textbf{Other baseline training variants for comparison}} & \multicolumn{2}{c}{P+R} & \multicolumn{2}{c}{P+A} & \\ 
\hline
 \multicolumn{2}{l|}{BERT original} &\multicolumn{1}{c}{} & \multicolumn{2}{c|}{72.65} & \multicolumn{3}{c}{58.10} &\\
\multicolumn{2}{l|}{RUBER pretrained on only Reddit} &\multicolumn{1}{c}{}& \multicolumn{2}{c|}{72.18} & \multicolumn{3}{c}{55.75} &\\
\multicolumn{2}{l|}{DEB pretrained on only Reddit} &\multicolumn{1}{c}{}& \multicolumn{2}{c|}{84.16} & \multicolumn{3}{c}{59.82} &\\
%BERT original & 72.65  & 58.10 \\
%DEB pretrained on Reddit & 84.16 & 59.82
%      RUBER pretrained on Reddit & 72.18  & 55.75 \\ 

\end{tabular}}
\caption{Performance of models based on the different training schemes. The accuracies are reported on the test set of DialyDialog++ on two types: Best accuracies for each training method are in \textcolor{red}{red} for classifying Positive responses from Random negatives and \textcolor{blue}{blue} for distinguishing Positive responses from Adversarial negatives.}
\label{tab:accuracies}
\end{table*}

==> tmp.tex <==
\section{Experiments}

\subsection{Evaluation on Random Negatives}
1. n-gram and word embedding methods are bd
2. ADEM and RUBER are better
3. DEB is the sota 

ADEM is bad, thereby use RUBER and DEB for further studies

explain boxplots, 25-75 interval, inliers, outliers, 

\subsection{Ablation study of DEB}
kind of ablation study
1. BERT with original pre-training 
2. BERT with Reddit pre-train
3. with finetune on random negs

\subsection{Hand Crafted Attacks}
1. RUBER and DEB results
2. DEB is superior to RUBER - better robustness 

by human judgements 
and observations 

\subsection{Adversarial Evaluation on DailyDialog++}
1. ADEM, RUBER, DEB are bad.  - put confusion matrix on trained on rand negs - put acc & pbc nos only (no box plot)
2. say if it's trained on both eg, it improves - just pbc & acc numbers 

\subsection{Exploring Diff losses}

1. Triplet loss (adversarial)
2. Hinge Loss

\subsection{Conicity}

try to understand why adv negs might be difficult 

pretrained DEB - positives and adv negs are very close, but rand neg are far 
use conicity diagrams 

however, when adv negs are inc in train both pos and adv negs are sep 

\subsection{Integrated gradients}
 brief intro
 - put plots to explain the fact that the model is getting confused by words in common with the context for adv negs. 
 
 - if there are some other intesting plots, pls add

